Neural Radiance Field Codebooks

Compositional representations of the world are a promising step towards enabling high-level scene understanding and efficient transfer to downstream tasks. Learning such representations for complex scenes and tasks remains an open challenge. Towards this goal, we introduce Neural Radiance Field Codebooks (NRC), a scalable method for learning object-centric representations through novel view reconstruction. NRC learns to reconstruct scenes from novel views using a dictionary of object codes which are decoded through a volumetric renderer. This enables the discovery of reoccurring visual and geometric patterns across scenes which are transferable to downstream tasks. We show that NRC representations transfer well to object navigation in THOR, outperforming 2D and 3D representation learning methods by 3.1% success rate. We demonstrate that our approach is able to perform unsupervised segmentation for more complex synthetic (THOR) and real scenes (NYU Depth) better than prior methods (29% relative improvement). Finally, we show that NRC improves on the task of depth ordering by 5.5% accuracy in THOR.

==> iclr2023/09_Reproducibility.tex <==
\section*{Reproducibility}
We include our code in the supplementary material. Hyper-parameters and implementation details for reproducing experiments can be found in Appendix \ref{app:implementation}. Details for evaluation procedures and datasets can be found in Section \ref{sec:experiments} and Appendix \ref{App:datasets}.

==> iclr2023/Figures/FailureAnalysis.tex <==
\begin{figure}[t!]
  \centering
  \makebox[\columnwidth][l]{\includegraphics[width=1\textwidth]{iclr2023/Figures/Codes_Fig.pdf}}
  \caption{Place Holder}
  \label{app:failure_analysis}
\end{figure}
